Task inefficiency patterns for a wave equation solver

The orchestration of complex algorithms demands high levels of automation to use modern hardware efficiently. Task-based programming with OpenMP 5.0 is a prominent candidate to accomplish this goal. We study OpenMP 5.0's tasking in the context of a wave equation solver (ExaHyPE) using three different architectures and runtimes. We describe several task-scheduling flaws present in currently available runtimes, demonstrate how they impact performance and show how to work around them. Finally, we propose extensions to the OpenMP standard.

==> 05d_merge.tex <==
\subsection{Task merging}

%
% Problem
%
We spawn many ready tasks in one go and rely on the OpenMP runtime to
distribute these tasks efficiently among the available cores.  With OpenMP 5,
we furthermore reserve the right to deploy tasks to GPGPUs.  This induces two
problems: First, our performance suffers from the overhead we produce by
launching thousands of GPGPU kernels.  Second, our GPU task implementations
require us to equip kernels with \texttt{omp parallel for} statements such that
the GPU thread teams are exploited efficiently.  Simultaneously, the same
kernel launched within a CPU task is bound to one core and the
\texttt{parallel} statement thus only induces overhead.

\begin{feature}
 It would help if we could extend single OpenMP tasks to multiple CPU cores.
\end{feature}

\noindent
We have, so far, not succeeded in realising this feature on top of OpenMP.
Consequently, we risk that a manycore chip is underutilised once the runtime is
confronted with only a few expensive enclave tasks.


\begin{feature}
It would help if the OpenMP runtime could fuse multiple ready tasks
simultaneously and launch them through one overarching texttt{parallel for}
(on an accelerator).
\end{feature}


\noindent
In our code, we realise this pattern within $\textsc{processPendingTasks}$: By
default, half of the pending tasks are processed before we check the
\texttt{while} loop again.  In another variation of our code, we introduce a
maximum number of sets of tasks to deploy to a GPU during a single BSP-type
sweep.  Until this threshold is met, we merge all pending tasks of the same
type in $\textsc{processPendingTasks}$ manually and deploy them as separate
OpenMP offloading tasks, which internally loop over this set of tasks with one
large \texttt{parallel for} on the GPU.

\marginpar{cite \cite{Iwasaki:2019:UserLevelThreads} somewhere here}
Offloading requires reasonably intense tasks, which is somewhat orthogonal to
tasking, where a lot of the efficiency is promised to be rooted in very
fine-grained concurrency.  Our approach allows OpenMP to fuse tasks of the same
type, deploy them as one chunk to an accelerator to process them there en bloc.
The runtime can thus balance on-node concurrency and offloading efficiency.
The fundamental problem behind such an approach is that it requires manual task
annotation (task type), a manual fusion of tasks (meta tasks to accommodate
multiple original tasks), and threshold parameters (how many tasks should
minimally be deployed to a GPU or how many task assemblies should occur at
most).  We are therefore faced with a hyperparameter optimisation challenge.

